Multimodal Deep Learning

This book is the result of a seminar in which we reviewed multimodal approaches and attempted to create a solid overview of the field, starting with the current state-of-the-art approaches in the two subfields of Deep Learning individually. Further, modeling frameworks are discussed where one modality is transformed into the other, as well as models in which one modality is utilized to enhance representation learning for the other. To conclude the second part, architectures with a focus on handling both modalities simultaneously are introduced. Finally, we also cover other modalities as well as general-purpose multi-modal models, which are able to handle different tasks on different modalities within one unified architecture. One interesting application (Generative Art) eventually caps off this booklet.

==> Makefile <==
ENGINE    = pdflatex
BIBENGINE = bibtex
FILE      = book
MAKE      = make

.PHONY: all clean compile bcompile

all:
	@$(MAKE) --no-print-directory clean
	@$(MAKE) --no-print-directory compile || true
	@$(MAKE) --no-print-directory bcompile
	@$(MAKE) --no-print-directory compile
	@$(MAKE) --no-print-directory compile
	@$(MAKE) --no-print-directory clean

clean:
	@rm "$(FILE).aux" \
 	    "$(FILE).log" \
 		  "$(FILE).toc" \
 		  "$(FILE).blg" \
 		  "$(FILE).lof" \
 		  "$(FILE).lot" \
 		  "$(FILE).out" \
 		  "$(FILE).idx" \
 		  "$(FILE).dvi"  || true

compile:
	$(ENGINE) "$(FILE).tex"

bcompile:
	$(BIBENGINE) "$(FILE).aux"

